Investigating Techniques to Optimise the Layout of Turbines in a Windfarm using a Quantum Computer

This paper investigates Windfarm Layout Optimization (WFLO), where we formulate turbine placement considering wake effects as a Quadratic Unconstrained Binary Optimization (QUBO) problem. Wind energy plays a critical role in the transition toward sustainable power systems, but the optimal placement of turbines remains a challenging combinatorial problem due to complex wake interactions. With recent advances in quantum computing, there is growing interest in exploring whether hybrid quantum-classical methods can provide advantages for such computationally intensive tasks. We investigate solving the resulting QUBO problem using the Variational Quantum Eigensolver (VQE) implemented on Qiskit's quantum computer simulator, employing a quantum noise-free, gate-based circuit model. Three classical optimizers are discussed, with a detailed analysis of the two most effective approaches: Constrained Optimization BY Linear Approximation (COBYLA) and Bayesian Optimization (BO). We compare these simulated quantum results with two established classical optimization methods: Simulated Annealing (SA) and the Gurobi solver. The study focuses on 4$\times$4 grid configurations (requiring 16 qubits), providing insights into near-term quantum algorithm applicability for renewable energy optimization.

==> Definitions/journalnames.tex <==
% Updated 18 December 2024 used for Y2025
%% --------------------------------------------------------------------
%\DeclareOption{}{%%
%		\gdef\@journal{}
%		\gdef\@journalfull{}
%		\gdef\@journalshort{}
%		\gdef\@doiabbr{}
%		\gdef\@ISSN{}
%		\gdef\@continuouspages{yes}
%		\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalshort: Short Name (ISO4)
%% - @journalfull: Journal full name
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.32604/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use 	\gdef\@continuouspages{yes} for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{biocell}{%
	\gdef\@journal{biocell}
	\gdef\@journalshort{Biocell}
	\gdef\@journalfull{Biocell}
	\gdef\@doiabbr{biocell}
	\gdef\@ISSN{1667-5746}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{chd}{%
	\gdef\@journal{chd}
	\gdef\@journalshort{Congenit Heart Dis}
	\gdef\@journalfull{Congenital Heart Disease}
	\gdef\@doiabbr{chd}
	\gdef\@ISSN{1747-0803}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmc}{%
 	\gdef\@journal{cmc}
	\gdef\@journalshort{Comput Mater Contin.}
	\gdef\@journalfull{Computers, Materials \& Continua}
	\gdef\@doiabbr{cmc}	\gdef\@ISSN{1546-2226}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{cmes}{%
 	\gdef\@journal{cmes}
	\gdef\@journalshort{Comput Model Eng Sci}
	\gdef\@journalfull{Computer Modeling in Engineering \& Sciences}
	\gdef\@doiabbr{cmes}
	\gdef\@ISSN{1526-1506}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{csse}{%
 	\gdef\@journal{csse}
	\gdef\@journalshort{Comput Syst Sci Eng}
	\gdef\@journalfull{Computer Systems Science and Engineering}
	\gdef\@doiabbr{csse}
	\gdef\@ISSN{0267-6192}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{dedt}{%
 	\gdef\@journal{dedt}
	\gdef\@journalshort{Digit Eng Digit Twin}
	\gdef\@journalfull{Digital Engineering and Digital Twin}
	\gdef\@doiabbr{dedt}
	\gdef\@ISSN{ }
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{ee}{%
 	\gdef\@journal{ee}
	\gdef\@journalshort{Energy Eng}
	\gdef\@journalfull{Energy Engineering}
	\gdef\@doiabbr{ee}
	\gdef\@ISSN{1546-0118}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fdmp}{%
 	\gdef\@journal{fdmp}
	\gdef\@journalshort{Fluid Dyn Mater Process}
	\gdef\@journalfull{Fluid Dynamics \& Materials Processing}
	\gdef\@doiabbr{fdmp}
	\gdef\@ISSN{1555-2578}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{fhmt}{%
 	\gdef\@journal{fhmt}
	\gdef\@journalshort{Front Heat Mass Transf}
	\gdef\@journalfull{Frontiers in Heat and Mass Transfer}
	\gdef\@doiabbr{fhmt}
	\gdef\@ISSN{2125-8629}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{iasc}{%
 	\gdef\@journal{iasc}
	\gdef\@journalshort{Intell Autom Soft Comput}
	\gdef\@journalfull{Intelligent Automation \& Soft Computing}
	\gdef\@doiabbr{iasc}
	\gdef\@ISSN{2326-005X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{icces}{%
 	\gdef\@journal{icces}
	\gdef\@journalshort{Int Conf Comput Exp Eng Sci}
	\gdef\@journalfull{The International Conference on Computational \& Experimental Engineering and Sciences}
	\gdef\@doiabbr{icces}
	\gdef\@ISSN{1993-2815}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{ijmhp}{%
 	\gdef\@journal{ijmhp}
	\gdef\@journalshort{Int J Ment Health Promot}
	\gdef\@journalfull{International Journal of Mental Health Promotion}
	\gdef\@doiabbr{ijmhp}
	\gdef\@ISSN{2049-8543}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jai}{%
 	\gdef\@journal{jai}
	\gdef\@journalshort{J Artif Intell}
	\gdef\@journalfull{Journal on Artificial Intelligence}
	\gdef\@doiabbr{jai}
	\gdef\@ISSN{2579-003X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jbd}{%
 	\gdef\@journal{jbd}
	\gdef\@journalshort{J Big Data}
	\gdef\@journalfull{Journal on Big Data}
	\gdef\@doiabbr{jbd}
	\gdef\@ISSN{2579-0056}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jbic}{%
 	\gdef\@journal{jbic}
	\gdef\@journalshort{J Blockchain Intell Comput}
	\gdef\@journalfull{Journal of Blockchain and Intelligent Computing}
	\gdef\@doiabbr{jbic}
	\gdef\@ISSN{}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{jcs}{%
 	\gdef\@journal{jcs}
	\gdef\@journalshort{J Cyber Secur}
	\gdef\@journalfull{Journal of Cyber Security}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2579-0064}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jihpp}{%
 	\gdef\@journal{jihpp}
	\gdef\@journalshort{J Inf Hiding Priv Prot}
	\gdef\@journalfull{Journal of Information Hiding and Privacy Protection}
	\gdef\@doiabbr{jihpp}
	\gdef\@ISSN{2637-4226}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jimh}{%
 	\gdef\@journal{jimh}
	\gdef\@journalshort{JIMH}
	\gdef\@journalfull{Journal of Intelligent Medicine and Healthcare}
	\gdef\@doiabbr{jimh}
	\gdef\@ISSN{2837-634X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jiot}{%
 	\gdef\@journal{jiot}
	\gdef\@journalshort{J Internet Things}
	\gdef\@journalfull{Journal on Internet of Things}
	\gdef\@doiabbr{jiot}
	\gdef\@ISSN{2579-0080}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jnm}{%
 	\gdef\@journal{jnm}
	\gdef\@journalshort{J New Media}
	\gdef\@journalfull{Journal of New Media}
	\gdef\@doiabbr{jnm}
	\gdef\@ISSN{2579-0129}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
 	\gdef\@journal{jpm}
	\gdef\@journalshort{J Polym Mater}
	\gdef\@journalfull{Journal of Polymer Materials}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{0976-3449}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jqc}{%
 	\gdef\@journal{jqc}
	\gdef\@journalshort{J Quantum Comput}
	\gdef\@journalfull{Journal of Quantum Computing}
	\gdef\@doiabbr{jqc}
	\gdef\@ISSN{2579-0145}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{jrm}{%
 	\gdef\@journal{jrm}
	\gdef\@journalshort{J Renew Mater}
	\gdef\@journalfull{Journal of Renewable Materials}
	\gdef\@doiabbr{jrm}
	\gdef\@ISSN{2164-6341}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{or}{%
 	\gdef\@journal{or}
	\gdef\@journalshort{Oncol Res}
	\gdef\@journalfull{Oncology Research}
	\gdef\@doiabbr{or}
	\gdef\@ISSN{1555-3906}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{phyton}{%
 	\gdef\@journal{phyton}
	\gdef\@journalshort{Phyton-Int J Exp Bot}
	\gdef\@journalfull{Phyton-International Journal of Experimental Botany}
	\gdef\@doiabbr{phyton}
	\gdef\@ISSN{1851-5657}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{po}{%
 	\gdef\@journal{po}
	\gdef\@journalshort{Psycho-Oncologie}
	\gdef\@journalfull{Psycho-Oncologie}
	\gdef\@doiabbr{po}
	\gdef\@ISSN{1778-381X}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{rig}{%
 	\gdef\@journal{rig}
	\gdef\@journalshort{Rev Int Géomatique}
	\gdef\@journalfull{Revue Internationale de Géomatique}
	\gdef\@doiabbr{rig}
	\gdef\@ISSN{2116-7060}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sdhm}{%
 	\gdef\@journal{sdhm}
	\gdef\@journalshort{Struct Durab Health Monit}
	\gdef\@journalfull{Structural Durability \& Health Monitoring}
	\gdef\@doiabbr{sdhm}
	\gdef\@ISSN{1930-2991}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{sv}{%
 	\gdef\@journal{sv}
	\gdef\@journalshort{Sound Vib}
	\gdef\@journalfull{Sound \& Vibration}
	\gdef\@doiabbr{sv}
	\gdef\@ISSN{2693-1443}
	\gdef\@continuouspages{yes}
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{journal}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{TEST}
	\gdef\@journalshort{TEST}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}

==> Definitions/package.tex <==
%%%%Update on 30 November 2023%%%
\usepackage[normalem]{ulem} % For using the command \uuline{} in the \abstract 
\usepackage{amsfonts} % Use for some special math mark
%%\usepackage{pxfonts} % Use for some special math mark 
%\usepackage{wasysym} % Use for some special mark
%\usepackage{subfigure} % For some paper the use \subfigure
\usepackage{mathcomp} % For permille mark
\usepackage{CJKutf8} % For Chinese font
\usepackage{pifont} % For some special mark 
\usepackage{bm} % Forr math enviroment bold format
\usepackage{bbm} % For some math fancy characters
\graphicspath{{./Definitions/}} % Use for import path the figures paper used


\makeatletter
\def\T@n@@nc@d@ngM@cr@M@d{}
\def\LY@n@@nc@d@ngM@cr@M@d{}
\makeatother

%\let\orignewcommand\newcommand  % Store the original \newcommand
%\let\newcommand\providecommand  % Make \newcommand behave like \providecommand
\usepackage{verse}
\let\newcommand\orignewcommand  % Use the original `\newcommand` in future
\makeatletter
\renewcommand*{\theHpoemline}{\arabic{verse@envctr}.\arabic{poemline}} % Use the original definition from verse.sty
\makeatother

% Define a matrix envrioment
\newsavebox\foobox
\newcommand{\slantbox}[2][.2]{\mbox{%
        \sbox{\foobox}{#2}%
        \hskip\wd\foobox
        \pdfsave
        \pdfsetmatrix{1 0 #1 1}%
        \llap{\usebox{\foobox}}%
        \pdfrestore
}}

%\setlength{\fboxsep}{0cm}

% Define triangledown mark
\let\oldblacktriangledown\blacktriangledown

% Define \dagger using unicode
\renewcommand{\dagger}{\mathchar"2279}
\renewcommand{\ddagger}{\mathchar"227A}

% Define italic In, Max
\newcommand{\mmathit}[1]{
  \ifthenelse{\equal{#1}{\ln}}{\mathit{ln}}{
    \ifthenelse{\equal{#1}{\max}}{\mathit{max}}{\mathit{#1}}
  }
}
\makeatother
\robustify{\footnote}

==> Definitions/packageHack.tex <==
%%%%Update on 30 November 2023%%%
\makeatletter
\usepackage[normalem]{ulem} % For \uuline and \st
\usepackage{amsfonts} 
\usepackage{mathcomp} % For permille mark
\usepackage{CJKutf8} % For Chinese font
\usepackage{pifont} % For special symbols
\usepackage{bm} % For bold math
\usepackage{bbm} % For math blackboard characters
\usepackage{etoolbox} % For boolean toggles
\usepackage{verse}

% Safe matrix environment

% === Untracked ==
\renewcommand{\sout}[1]{}
\newcommand{\corr}[1]{\textcolor{black}{#1}}
\newcommand{\Corr}[3]{\textcolor{black}{#1}}

% === Tracked ==
%\newcommand{\Corr}[3]{\textcolor{red}{#1 [Changes in this section were made per Reviewer #2, Question #3]}}
%\newcommand{\corr}[1]{\textcolor{red}{#1}}

\newsavebox\foobox
\newcommand{\slantbox}[2][.2]{\mbox{%
        \sbox{\foobox}{#2}%
        \hskip\wd\foobox
        \pdfsave
        \pdfsetmatrix{1 0 #1 1}%
        \llap{\usebox{\foobox}}%
        \pdfrestore
}}

% Math italics for special functions
\newcommand{\mmathit}[1]{%
  \ifstrequal{#1}{\ln}{\mathit{ln}}{%
    \ifstrequal{#1}{\max}{\mathit{max}}{%
      \ifstrequal{#1}{\log}{\mathit{log}}{%
        \mathit{#1}%
      }%
    }%
  }%
}

% Robust footnotes early
\robustify{\footnote}

% Special symbol redefinitions
\renewcommand{\dagger}{\mathchar"2279}
\renewcommand{\ddagger}{\mathchar"227A}
\let\oldblacktriangledown\blacktriangledown

% Graphics path
\graphicspath{{./Definitions/}}
\makeatother



==> Definitions/unicode.tex <==

\DeclareUnicodeCharacter{1E45}{\.{n}}
\DeclareUnicodeCharacter{1E41}{\.{m}}
\DeclareUnicodeCharacter{2003}{\quad}
%\DeclareUnicodeCharacter{0177}{\^{y}}
%\DeclareUnicodeCharacter{101}{\={a}}
\DeclareUnicodeCharacter{2009}{\thinspace}
\DeclareUnicodeCharacter{2002}{\enspace{}}
\DeclareUnicodeCharacter{2005}{\thinspace}
\DeclareUnicodeCharacter{0263}{\textipa{G}}
%\DeclareUnicodeCharacter{117}{\.{e}}
\DeclareUnicodeCharacter{A0}{~}
\DeclareUnicodeCharacter{2460}{\textcircled{\scriptsize{1}}}
\DeclareUnicodeCharacter{2461}{\textcircled{\scriptsize{2}}}
\DeclareUnicodeCharacter{2462}{\textcircled{\scriptsize{3}}}
\DeclareUnicodeCharacter{2463}{\textcircled{\scriptsize{4}}}
\DeclareUnicodeCharacter{2464}{\textcircled{\scriptsize{5}}}
\DeclareUnicodeCharacter{2465}{\textcircled{\scriptsize{6}}}
\DeclareUnicodeCharacter{2466}{\textcircled{\scriptsize{7}}}
\DeclareUnicodeCharacter{2467}{\textcircled{\scriptsize{8}}}
\DeclareUnicodeCharacter{2468}{\textcircled{\scriptsize{9}}}
\DeclareUnicodeCharacter{2070}{\textsuperscript{0}}
\DeclareUnicodeCharacter{2074}{\textsuperscript{4}}
\DeclareUnicodeCharacter{2075}{\textsuperscript{5}}
\DeclareUnicodeCharacter{2076}{\textsuperscript{6}}
\DeclareUnicodeCharacter{2077}{\textsuperscript{7}}
\DeclareUnicodeCharacter{2078}{\textsuperscript{8}}
\DeclareUnicodeCharacter{2079}{\textsuperscript{9}}
\DeclareUnicodeCharacter{02C2}{<}
\DeclareUnicodeCharacter{2033}{\relax\ifmmode '' \else $''$\fi}
\DeclareUnicodeCharacter{2034}{\relax\ifmmode ''' \else $'''$\fi}
\DeclareUnicodeCharacter{2026}{\relax\ifmmode … \else $\ldots$\fi}
\DeclareUnicodeCharacter{0229}{\c{e}}
\DeclareUnicodeCharacter{016F}{\r{u}}
%\DeclareUnicodeCharacter{0218}{\cb{S}}
%\DeclareUnicodeCharacter{0219}{\cb{s}}
%\DeclareUnicodeCharacter{021B}{\cb{t}}
\DeclareUnicodeCharacter{127}{\relax\ifmmode\rm\hbar\else $\rm\hbar$\fi}
\DeclareUnicodeCharacter{3AC}{\relax\ifmmode\acute{\alpha}\else $\acute{\alpha}$\fi}
\DeclareUnicodeCharacter{3AD}{\relax\ifmmode\acute{\varepsilon}\else $\acute{\varepsilon}$\fi}
\DeclareUnicodeCharacter{3AE}{\relax\ifmmode\acute{\eta}\else $\acute{\eta}$\fi}
\DeclareUnicodeCharacter{3AF}{\relax\ifmmode\acute{\iota}\else $\acute{\iota}$\fi}
\DeclareUnicodeCharacter{3CC}{\relax\ifmmode\acute{o}\else $\acute{o}$\fi}
\DeclareUnicodeCharacter{3CD}{\relax\ifmmode\acute{\upsilon}\else $\acute{\upsilon}$\fi}
\DeclareUnicodeCharacter{3CE}{\relax\ifmmode\acute{\omega}\else $\acute{\omega}$\fi}
\DeclareUnicodeCharacter{391}{A}
\DeclareUnicodeCharacter{392}{B}
\DeclareUnicodeCharacter{395}{E}
\DeclareUnicodeCharacter{396}{Z}
\DeclareUnicodeCharacter{397}{H}
\DeclareUnicodeCharacter{399}{I}
\DeclareUnicodeCharacter{39A}{K}
\DeclareUnicodeCharacter{39C}{M}
\DeclareUnicodeCharacter{39D}{N}
\DeclareUnicodeCharacter{39F}{O}
\DeclareUnicodeCharacter{3A1}{P}
\DeclareUnicodeCharacter{3A4}{T}
\DeclareUnicodeCharacter{3A7}{X}

\DeclareUnicodeCharacter{27E6}{\relax\ifmmode \llbracket \else $\llbracket$\fi}
\DeclareUnicodeCharacter{27E7}{\relax\ifmmode \rrbracket \else $\rrbracket$\fi}

\DeclareUnicodeCharacter{1D434}{\relax\ifmmode A \else $A$\fi}
\DeclareUnicodeCharacter{1D435}{\relax\ifmmode B \else $B$\fi}
\DeclareUnicodeCharacter{1D436}{\relax\ifmmode C \else $C$\fi}
\DeclareUnicodeCharacter{1D437}{\relax\ifmmode D \else $D$\fi}
\DeclareUnicodeCharacter{1D438}{\relax\ifmmode E \else $E$\fi}
\DeclareUnicodeCharacter{1D439}{\relax\ifmmode F \else $F$\fi}
\DeclareUnicodeCharacter{1D43A}{\relax\ifmmode G \else $G$\fi}
\DeclareUnicodeCharacter{1D43B}{\relax\ifmmode H \else $H$\fi}
\DeclareUnicodeCharacter{1D43C}{\relax\ifmmode I \else $I$\fi}
\DeclareUnicodeCharacter{1D43D}{\relax\ifmmode J \else $J$\fi}
\DeclareUnicodeCharacter{1D43E}{\relax\ifmmode K \else $K$\fi}
\DeclareUnicodeCharacter{1D43F}{\relax\ifmmode L \else $L$\fi}
\DeclareUnicodeCharacter{1D440}{\relax\ifmmode M \else $M$\fi}
\DeclareUnicodeCharacter{1D441}{\relax\ifmmode N \else $N$\fi}
\DeclareUnicodeCharacter{1D442}{\relax\ifmmode O \else $O$\fi}
\DeclareUnicodeCharacter{1D443}{\relax\ifmmode P \else $P$\fi}
\DeclareUnicodeCharacter{1D444}{\relax\ifmmode Q \else $Q$\fi}
\DeclareUnicodeCharacter{1D445}{\relax\ifmmode R \else $R$\fi}
\DeclareUnicodeCharacter{1D446}{\relax\ifmmode S \else $S$\fi}
\DeclareUnicodeCharacter{1D447}{\relax\ifmmode T \else $T$\fi}
\DeclareUnicodeCharacter{1D448}{\relax\ifmmode U \else $U$\fi}
\DeclareUnicodeCharacter{1D449}{\relax\ifmmode V \else $V$\fi}
\DeclareUnicodeCharacter{1D44A}{\relax\ifmmode W \else $W$\fi}
\DeclareUnicodeCharacter{1D44B}{\relax\ifmmode X \else $X$\fi}
\DeclareUnicodeCharacter{1D44C}{\relax\ifmmode Y \else $Y$\fi}
\DeclareUnicodeCharacter{1D44D}{\relax\ifmmode Z \else $Z$\fi}
\DeclareUnicodeCharacter{1D44E}{\relax\ifmmode a \else $a$\fi}
\DeclareUnicodeCharacter{1D44F}{\relax\ifmmode b \else $b$\fi}
\DeclareUnicodeCharacter{1D450}{\relax\ifmmode c \else $c$\fi}
\DeclareUnicodeCharacter{1D451}{\relax\ifmmode d \else $d$\fi}
\DeclareUnicodeCharacter{1D452}{\relax\ifmmode e \else $e$\fi}
\DeclareUnicodeCharacter{1D453}{\relax\ifmmode f \else $f$\fi}
\DeclareUnicodeCharacter{1D454}{\relax\ifmmode g \else $g$\fi}
\DeclareUnicodeCharacter{1D456}{\relax\ifmmode i \else $i$\fi}
\DeclareUnicodeCharacter{1D457}{\relax\ifmmode j \else $j$\fi}
\DeclareUnicodeCharacter{1D458}{\relax\ifmmode k \else $k$\fi}
\DeclareUnicodeCharacter{1D459}{\relax\ifmmode l \else $l$\fi}
\DeclareUnicodeCharacter{1D45A}{\relax\ifmmode m \else $m$\fi}
\DeclareUnicodeCharacter{1D45B}{\relax\ifmmode n \else $n$\fi}
\DeclareUnicodeCharacter{1D45C}{\relax\ifmmode o \else $o$\fi}
\DeclareUnicodeCharacter{1D45D}{\relax\ifmmode p \else $p$\fi}
\DeclareUnicodeCharacter{1D45E}{\relax\ifmmode q \else $q$\fi}
\DeclareUnicodeCharacter{1D45F}{\relax\ifmmode r \else $r$\fi}
\DeclareUnicodeCharacter{1D460}{\relax\ifmmode s \else $s$\fi}
\DeclareUnicodeCharacter{1D461}{\relax\ifmmode t \else $t$\fi}
\DeclareUnicodeCharacter{1D462}{\relax\ifmmode u \else $u$\fi}
\DeclareUnicodeCharacter{1D463}{\relax\ifmmode v \else $v$\fi}
\DeclareUnicodeCharacter{1D464}{\relax\ifmmode w \else $w$\fi}
\DeclareUnicodeCharacter{1D465}{\relax\ifmmode x \else $x$\fi}
\DeclareUnicodeCharacter{1D466}{\relax\ifmmode y \else $y$\fi}
\DeclareUnicodeCharacter{1D467}{\relax\ifmmode z \else $z$\fi}

\DeclareUnicodeCharacter{1E67}{\.{\v s}}
\DeclareUnicodeCharacter{1E11}{\relax\ifmmode \c{d} \else $\c{d}$\fi}
\DeclareUnicodeCharacter{1ECB}{\relax\ifmmode \d{i} \else $\d{i}$\fi}
\DeclareUnicodeCharacter{1D8D}{\relax\ifmmode \textlhookx \else $\textlhookx$\fi}
\DeclareUnicodeCharacter{104}{\relax\ifmmode \k{A} \else $\k{A}$\fi}
\DeclareUnicodeCharacter{211E}{\relax\ifmmode \textrecipe \else $\textrecipe$\fi}
\DeclareUnicodeCharacter{29D}{\relax\ifmmode \textctj \else $\textctj$\fi}

\DeclareUnicodeCharacter{1E2E}{\'{\"I}}
\DeclareUnicodeCharacter{23F}{\textrts}

\DeclareUnicodeCharacter{2C73}{\varw}

\DeclareUnicodeCharacter{2127}{\mho}

\DeclareUnicodeCharacter{28C}{\textturnv}
\DeclareUnicodeCharacter{252}{\textturnscripta}
\DeclareUnicodeCharacter{259}{\schwa}
\DeclareUnicodeCharacter{25B}{\m{e}}
\DeclareUnicodeCharacter{266}{\m{h}}
\DeclareUnicodeCharacter{127}{\B{h}}
\DeclareUnicodeCharacter{27E}{\textfishhookr}
\DeclareUnicodeCharacter{281}{\textinvscr}


